Domain Decomposition Method for Poisson--Boltzmann Equations based on Solvent Excluded Surface

In this paper, we develop a domain decomposition method for the nonlinear Poisson-Boltzmann equation based on a solvent-excluded surface widely used in computational chemistry. The model relies on a nonlinear equation defined in $\mathbb{R}^3$ with a space-dependent dielectric permittivity and an ion-exclusion function that accounts for steric effects. Potential theory arguments transform the nonlinear equation into two coupled equations defined in a bounded domain. Then, the Schwarz decomposition method is used to formulate local problems by decomposing the cavity into overlapping balls and only solving a set of coupled sub-equations in each ball. The main novelty of the proposed method is the introduction of a hybrid linear-nonlinear solver used to solve the equation. A series of numerical experiments are presented to test the method and show the importance of the nonlinear model.

==> discretisation.tex <==
In the previous section we presented a solution for the HSP equation and the GSP equation in an unit sphere. Here, we define them on a generalised domain $\Omega_i$ for any $i\in \lbrace 1,\dots, M\rbrace$ and also present the discretisation of the coupling condition.

\subsection{Reformulation}
We first introduce some notations that will be used in this section. Let $\chi_i(\cdot)$ be the characteristic function of $\Omega_i$, i.e.,
\begin{equation*}
\chi_i(\bx):=\left\lbrace\begin{array}{ll}
1&\mathrm{if}\ \ \bx\in \Omega_i,\\
0&\mathrm{else,}
\end{array}\right.
\end{equation*}
then define
$$
\omega_{ji}(\bx):=\frac{\chi_i(\bx)}{|\mathcal{N}(j,\bx)|}=\frac{\chi_i(\bx)}{\sum_{k\neq j}\chi_k(\bx)}\quad \forall\bx\in \Omega_j,
$$
where $\mathcal{N}(j,\bx)$ represent the index set of all spheres containing $\bx$. If $|\mathcal{N}(j,\bx)|=0$ (i.e., $\bx\in \Gamma_j^{\te}$) we define $\omega_{ji}(\bx)=0$ for all $i$. Furthermore we define a characteristic function for the boundary
\begin{equation*}
\chi_i^{\te}(\bx):=\left\lbrace\begin{array}{ll}
1&\mathrm{if}\ \ \bx\in \Gamma_i^{\te},\\
0&\mathrm{else,}
\end{array}\right.
\end{equation*}
which is equivalent to
$$
\chi_i^{\te}(\bx)=1-\sum_{k\neq i}\omega_{ik}(\bx)\quad \forall\bx\in \Gamma_i.
$$
It's clear from the last equation that we can define the characteristic function for the internal part of the boundary of $\Gamma_i$ as
$$
\chi_i^{\ti}(\bx) = \sum_{k\neq i}\omega_{ik}(\bx)\quad \forall\bx\in \Gamma_i.
$$

\subsubsection{Domain Decomposition Scheme}
We notice that we have two coupling conditions for the PB equations one for the reaction potential given by Eq.~\eqref{eq:ndr_bc} and the other for extended potential given by Eq.~\eqref{eq:hsp_bc}. We recast Eq.~\eqref{eq:ndr_bc} as
\begin{equation*}
\psi_{\mr}|_{\Gamma_j}(\bx)-\sum_{k\neq j}\omega_{jk}(\bx)\psi_{\mr}|_{\Omega_k}(\bx)=\chi_j^{\te}(\bx)\left( g(\bx)-\psi_0(\bx)\right)\quad\forall\ \bx\in \Gamma_j.
\end{equation*}
Similarly, Eq.~\eqref{eq:hsp_bc} is modified as
\begin{equation*}
\psi_{\me}|_{\Gamma_j}(\bx)-\sum_{k\neq j}\omega_{jk}(\bx)\psi_{\me}|_{\Omega_k}(\bx)=\chi_j^{\te}(\bx)g(\bx)\quad\ \forall\ \bx\in\Gamma_j.
\end{equation*}

\begin{remark} Alongwith the local coupling conditions we also have a global coupling condition given by Eq.~\eqref{eq:global_coupling} which involves the non-local operator $\mathcal{S}_{\Gamma_0}(\cdot)$. This kind of coupling also arise in the LPB equation presented in \cite{QSM19} and we follow the same ideas as presented in the paper to approximate this integral. As the integral is over the whole boundary $\Gamma_0$, we divide the integral over whole of $\Gamma_0$ to integrals over each sphere $\Gamma_i$, i.e.,
\begin{equation*}
g(\bx)=\sum_{i=1}^M\tilde{\mathcal{S}}_{\Gamma_i}\left[ \chi_i^{\te}\left(\partial_{\bn}\psi_{\me}-\partial_{\bn}\left(\psi_{\mr}+\psi_0\right)\right)(\bx)\right]\quad\forall\ \bx\in \Gamma_0,
\end{equation*}
where
$$
\tilde{\mathcal{S}}_{\Gamma_i}\sigma:=\int_{\Gamma_i}\frac{\exp\left(-\kappa|\bx-\by|\right)\sigma(\by)}{4\pi|\bx-\by|}d\by\quad\ \forall\ \bx\in\mathbb{R}^3,
$$
and $\sigma$ is an arbitrary function in $H^{-1/2}(\Gamma_i)$.
\end{remark}

\subsection{System of Equations}
We now discretise our equations and present the global system of equations that will be used in the numerical simulations.

\subsubsection{HSP Equations}
For each sphere $\Gamma_j$ we approximate the HSP equation solution $\psi_{\me}|_{\Gamma_j}$ by a linear combination of the spherical harmonics $\left\lbrace Y_{\ell}^m(\cdot)\right\rbrace$ with $0\leq \ell\leq \ell_{\max}$ and $-\ell\leq m\leq \ell$ as
$$
\psi_{\me}|_{\Gamma_j}(\bx_j+R_j\bs)=\sum_{\ell=0}^{\ell_{\max}}\sum_{m=-\ell}^{\ell}\left[X_{\me}\right]_{j\ell m}Y_{\ell}^m(\bs),\quad\bs\in \mathbb{S}^2,
$$
where $\left[X_{\me}\right]_{j\ell m}$ are the unknown coefficients of the $Y_{\ell}^m(\cdot)$ mode and for any point $\bx\in \Gamma_j$ we actually use its spherical coordinates $\bx=\bx_j+R_j\bs$ for $\bs\in \mathbb{S}^2$. From the HSP solver it is easy to deduce that
$$
\psi_{\me}|_{\Omega_i}(\bx_i+r\bs)=\sum_{\ell=0}^{\ell_{\max}}\sum_{m=-\ell}^{\ell}\left[X_{\me}\right]_{j\ell m}\frac{i_{\ell'}(r)}{i_{\ell'}(R_i)}Y_{\ell}^m(\bs),\quad 0\leq r\leq R_i,\quad\bs\in \mathbb{S}^2.
$$
The global system of equations have been derived for the HSP equation in \cite[Eq.~(78)]{QSM19}. For completeness we present the final equations. The linear system of equations corresponding to the above discretisation are given by
\begin{equation}\label{eq:linear_system_hsp}
\bB X_{\me}=\overline{\bG}_X,
\end{equation}
where $\bB$ is a matrix of size $M(\ell_{\max}+1)^2\times M(\ell_{\max}+1)^2$, $ X_{\me}$ is the solution vector for the extended potential of size $M(\ell_{\max}+1)^2$, and $\bG_X$ is the right-hand side of size $M(\ell_{\max}+1)^2$. The $(j\ell m)^{\ith}$ entry of $\bB X_{\me}$ and $\overline{\bG}_X$ is given by
\begin{equation*}
\left[\bB X_{\me}\right]_{j\ell m}=\left[ X_{\me}\right]_{j\ell m}-\sum_{i\neq j}\sum_{\ell' m'}\left(\sum_{n=1}^{N_{\leb}}\omega_n^{\leb}\omega_{ji}(\bx_j+R_j\bs_n)\frac{i_{\ell'}(R_{ijn})}{i_{\ell'}(R_i)}Y_{\ell'}^{m'}(\bs_{ijn})Y_{\ell}^m(\bs_n)\right)\left[ X_{\me}\right]_{i\ell' m'},
\end{equation*}
and
\begin{equation*}
\left[\overline{\bG}_X\right]_{j\ell m}=\sum_{n=1}^{N_{\leb}}\omega_n^{\leb}\chi_j^{\te}(\bx_j+R_j\bs_n)g(\bx_j+R_j\bs_n)Y_{\ell}^m(\bs_n).
\end{equation*}
In the above equations $(R_{ijn},\bs_{ijn})$ are the spherical coordinates associated with $\Gamma_i$ of the point $\bx_j+R_j\bs_n$ such that
$$
\bx_j+R_j\bs_n=\bx_i+R_{ijn}\bs_{ijn}\quad\mathrm{with}\quad \bs_{ijn}\in \mathbb{S}^2.
$$

\subsubsection{GSP Equations}
The approximation of the solution for the GSP equation follows the same idea as that of the HSP equation. Let $L_k(\cdot)$ denote a Legendre polynomial of order $k$, then we define the shifted Legendre polynomials by
$$
\tilde{L}_k(\rho)=L_k\left(\frac{2(\rho-\delta_j)}{R_j-\delta_j}-1\right),
$$
where $\delta_j=r_j/R_j\in(0,1)$ and $\delta_j\leq \rho\leq R_j$. The reaction potential for each sphere $\Gamma_j$ is given as a linear combination of $\left\lbrace \tilde{L}_k(\cdot){\ylmdash}(\cdot)\right\rbrace$ for $k'=1,\dots,N,\ell'=0,\dots,\ell_{\max},$ and $m=-\ell',\dots,\ell'$ by
$$
\psi_{\mr}|_{\Gamma_j}(\bx_j+R_j\bs)=\sum_{k'=1}^N\sum_{\ell'=0}^{\ell_{\max}}\sum_{m'=-\ell'}^{\ell'}\left[X_{\mr}\right]_{jk'}^{\ell'm'}\tilde{L}_{k'}(R_j){\ylmdash}(\bs),\quad \bs\in\mathbb{S}^2.
$$
From the coupling condition we have for $\bx_j+R_j\bs\in \Gamma_j$,
\begin{equation}\label{eq:intermediate_eq_1}
\psi_{\mr}|_{\Gamma_j}(\bx_j+R_j\bs)-\sum_{i\neq j}\omega_{ji}(\bx_j+R_j\bs)\psi_{\mr}|_{\Omega_i}(\bx_j+R_j\bs)=\chi_j^{\te}(\bx_j+R_j\bs)\left(g(\bx_j+R_j\bs)-\psi_0(\bx_j+R_j\bs)\right).
\end{equation}

Now we know from the unit ball discretisation that $\Omega_i$ is divided into two parts, $\mathcal{D}_i$ and $B_{\delta_i}(\bx_i)$. The term $\psi_{\mr}|_{\Omega_i}(\bx_j+R_j\bs)$ can be seen as an operator which takes the point $\bx_j+R_j\bs$ and depending on its location in $\Omega_i$ returns the solution vector. Now, we can express $\psi_{\mr}|_{\Omega_i}$ by
\begin{equation*}
\psi_{\mr}|_{\Omega_i}(\bx_i+r\bs)=\left\lbrace
\begin{array}{ll}
\sum_{k'=1}^N\sum_{\ell'=0}^{\ell_{\max}}\sum_{m'=-\ell'}^{\ell'}\left[X_{\mr}\right]_{ik'}^{\ell'm'}\tilde{L}_{k'}(r)\ylmdash(\bs)&\mathrm{if}\quad \delta_i\leq r\leq R_i,\\
\sum_{k'=1}^N\sum_{\ell'=0}^{\ell_{\max}}\sum_{m'=-\ell'}^{\ell'}\left[X_{\mr}\right]_{ik'}^{\ell'm'}\left(\dfrac{r}{\delta_i}\right)^{\ell'}\tilde{L}_{k'}(\delta_i)\ylmdash(\bs)&\mathrm{if}\quad 0\leq r\leq \delta_i.
\end{array}\right.
\end{equation*}
To get the system of equations we multiply Eq.~\eqref{eq:intermediate_eq_1} by the basis function $\tilde{L}_{k}(\cdot)Y_{\ell m}(\cdot)$ and integrate over $\mathbb{S}^2$. Now, the $(k\ell m)^{\ith}$ entry for the $j^{\ith}$ sphere of the first term in Eq.~\eqref{eq:intermediate_eq_1} is given by
$$
\left\langle \psi_{\mr}|_{\Gamma_j}\left(\bx_j+R_j\cdot\right),\tilde{L}_k(R_j)\ylm(\cdot)\right\rangle_{\mathbb{S}^2}=\sum_{k'=1}^N\left[ X_{\mr}\right]_{jk'}^{\ell m}\tilde{L}_{k'}(R_j)\tilde{L}_k(R_j).
$$
From the unit ball formulation the $(k\ell m)^{\ith}$ term of the $2^{\mathrm{nd}}$ component in Eq.~\eqref{eq:intermediate_eq_1} is given by
\begin{alignat*}{3}
\lefteqn{\omega_{ji}(\bx_j+R_j\bs)\psi_{\mr}|_{\Omega_i}(\bx_j+R_j\bs) = \left[\bA^iX_{\mr}\right]_{k\ell m}}\nonumber \\
&= & \sum_{k'=1}^N\sum_{\ell'=0}^{\ell_{\max}}\sum_{m'=-\ell'}^{\ell'}\Bigg{[}\int_{\mathcal{D}_i}\omega_{ji}(\bx_j+R_j\bs)\varepsilon(\bx_i+r\bs) \nabla\left(\tilde{L}_{k'}(r_{ij})\ylmdash(\bs_{ij})\right)\cdot \nabla \left(\tilde{L}_k(r)\ylm(\bs)\right)drd\bs\nonumber \\
&& +\kappa^2\varepsilon_s\int_{\mathcal{D}_i}\omega_{ji}(\bx_j+R_j\bs)\lambda(\bx_i+r\bs)\tilde{\mathcal{F}}(\overline{X}_r)\tilde{L}_{k'}(r_{ij})\ylmdash(\bs_{ij})\tilde{L}_k(r)\ylm(\bs)drd\bs\\
&&+\frac{\ell}{\delta_i}\int_{\partial B_{\delta_i}(\bx_i)}\omega_{ji}(\bx_j+R_j\bs)\tilde{L}_{k'}(\delta_i)\ylmdash(\bs_{ij}) \tilde{L}_k(\delta_i)\ylm(\bs)d\bs\Bigg{]}\left[X_{\mr}\right]_{ik'}^{\ell'm'},
\end{alignat*}
if  $\bx_j+R_j\bs\in \mathcal{D}_i$ where
$$
\bx_j+R_j\bs = \bx_i+r_{ij}\bs_{ij},
$$
and
$$
\left[\bA^iX_{\mr}\right]_{k\ell m} = \sum_{k'=1}^N\sum_{\ell'=0}^{\ell_{\max}}\sum_{m'=-\ell'}^{\ell'}\sum_{n=1}^{N_{\leb}}\omega_n^{\leb}\left(\frac{R_{ijn}}{\delta_i}\right)^{\ell'}\tilde{L}_{k'}(\delta_i)\tilde{L}_k(\delta_i)\ylmdash(\bs_{ijn})\ylm(\bs_n),
$$
if  $\bx_j+R_j\bs\in \partial B_{\delta_i}(\bx_i)$ where we used the Lebedev quadrature formula to approximate the integral.

The final term to approximate is the right-hand side in Eq.~\eqref{eq:intermediate_eq_1}. This follows the same approach as in HSP but with different dimension of the vector. For completeness the $(k\ell m)^{\ith}$ entry for $\Gamma_j$ is given by
$$
\left[\bG_{X}\right]_{k\ell m}^j=\sum_{n=1}^{N_{\leb}}\omega_n^{\leb}\chi_j^{\te}(\bx_j+R_j\bs_n)g(\bx_j+R_j\bs_n)\tilde{L}_k(R_j)\ylm(\bs_n),
$$
and
$$
\left[\bG_0\right]_{k\ell m}^j=-\sum_{n=1}^{N_{\leb}}\omega_n^{\leb}\chi_j^{\te}(\bx_j+R_j\bs_n)\psi_0(\bx_j+R_j\bs_n)\tilde{L}_k(R_j)\ylm(\bs_n).
$$
Hence for sphere $\Gamma_j$ we get a matrix $\bA^j$ of size $N(\ell_{\max}+1)^2\times N(\ell_{\max}+1)^2$ whose $(k\ell m)^{\ith}$ entry is given by
$$
\left[ \bA^jX_{\mr}\right]_{k\ell m}=\sum_{k'=1}^N\left[X_{\mr}\right]_{j\ell m}^{k'}\tilde{L}_{k'}(R_j)\tilde{L}_k(R_j)-\sum_{i\neq j}\left[\bA^i X_{\mr}\right]_{k\ell m}.
$$
Finally, collecting the entries for all spheres we get the matrix formulation
$$
\bA X_{\mr}=\bG_X+\bG_0,
$$
where $\bA$ is of size $MN(\ell_{\max}+1)^2\times MN(\ell_{\max}+1)^2$, and $X_{\mr},\bG_X,\bG_0$ are of size $MN(\ell_{\max}+1)^2$.

\begin{remark}
For $k=1,\dots,N$ the block vectors of $\bG_X$ are identical to $\overline{\bG}_X$, i.e.,
$$
\bG_X^i= \bG_X^j= \overline{\bG}_X\,\quad \mathrm{for}\ \ i\neq j,\quad i,j\in\left\lbrace 1, \dots,N\right\rbrace,
$$
i.e., the size of $\bG_X^i$ is $M\left(\ell_{\max}+1\right)^2$ for $i\in\left\lbrace 1,\dots,N\right\rbrace$.
\end{remark}

\subsubsection{Global Equations}
Finally, combining the HSP and GSP equations we get the system of equation by
\begin{equation*}
\begin{aligned}
\bA X_{\mr} & =  \bG_X+\bG_0\\
\bB X_{\me} & =  \overline{\bG}_X,
\end{aligned}
\end{equation*}
where $X_{\mr}$ and $ X_{\me}$ are unknown vector of the reaction and extended potential, respectively. 

We now present the matrix entries for $\overline{\bG}_X$ which depends on the global coupling condition $g(\cdot)$ which in turn depends on $\partial_{\bn}\psi_{\mr}$, $\partial_{\bn}\psi_{\me}$, and $\partial_{\bn} \psi_0$. We split $\overline{\bG}_X$ as
$$
\overline{\bG}_X=\overline{\bF}_0-\overline{\bC}_1X_{\mr}-\overline{\bC}_2X_{\me},
$$
where $\overline{\bF}_0,\overline{\bC}_1,$ and $\overline{\bC}_2$ depends on $\partial_{\bn}\psi_0$, $\partial_{\bn}\psi_{\mr},$ and $\partial_{\bn}\psi_{\me}$ respectively. For $\overline{\bF}_0$ and $\overline{\bC}_2$ the entries are exactly the same as for ddLPB in \cite{QSM19} and hence we do not derive them but provide the entries. In contrast for $\overline{\bC}_1$ we have a rectangular matrix of size $M\left(\ell_{\max}+1\right)^2\times MN\left(\ell_{\max}+1\right)^2$. The derivation for the entries of $\overline{\bC}_1$ remains the same but with an additional index.

The $(i\ell m,jk'\ell'm')^{\ith}$ entry of $\overline{\bC}_1$ is given by
\begin{align}\label{eq:definition_of_C1_matrix}
\left[ \overline{\bC}_1\right]_{i\ell m}^{jk'\ell'm'} & :=  \left( \sum_{n=1}^{N_{\leb}}\omega_n^{\leb}\chi_i^{\te}(\bx_i+R_i\bs_n)Y_{\ell m}(\bs_n)\left[\bQ\right]_{j\ell'm'}^{in}\tilde{L}_{k'}\left(R_j\right)\frac{\ell'}{R_j}\right),
\end{align}
and the $(i\ell m,j\ell'm')^{\ith}$ entry of $\overline{\bC}_2$ is given by,
\begin{align}\label{eq:definition_of_C2_matrix}
\left[ \overline{\bC}_2\right]_{i\ell m}^{j\ell'm'} & :=  -\left( \sum_{n=1}^{N_{\leb}}\omega_n \chi_i^{\te}(\bx_i+R_i\bs_n)Y_{\ell m}(\bs_n)\left[\bQ\right]_{j\ell'm'}^{in}\frac{\ti'_{\ell'}(R_j)}{\ti_{\ell'}(R_j)}\right),
\end{align}
where matrix $\bQ$ is  a matrix of size $M\left(\ell_{\max}+1\right)^2\times MN_{\leb}$ and the $(j\ell'm',in)^{\mathrm{th}}$ entry is given by
\begin{align}\label{eq:definition_of_Q_matrix}
\left[ \bQ\right]_{j\ell'm'}^{in} & :=  \sum_{\ell_0=0}^{\ell_{\max}}\sum_{m_0=-\ell_0}^{\ell_0}\cik \left[ \bP \chi_j^{\te}\right]_{\ell_0m_0}^{\ell'm'} \bk_{\ell_0}^j(\bx_i+R_i\bs_n)Y_{\ell_0m_0}^j(\bx_i+R_i\bs_n),
\end{align}
where 
$\bk_{\ell_0}^{j}(\bx)$ is defined by
\begin{equation}\label{eq:definition_of_bessel_func_second}
\bk_{\ell_0}^{j}(\bx)=\frac{\tk_{\ell_0}(|\bx-\bx_j|)}{\tk_{\ell_0}(R_j)},
\end{equation}
$\tk_{\ell_0}(\bx)$ is the modified spherical Bessel's function of the second kind,
$$
\cik=\left( \frac{\ti'_{\ell_0}(R_j)}{\ti_{\ell_0}(R_j)}-\frac{\tk'_{\ell_0}(R_j)}{\tk_{\ell_0}(R_j)}\right)^{-1},
$$ 
and $\ti_{\ell_0}(\bx)$ is the modified spherical Bessel's function of the first kind.

The matrix $\bP \chi_j^{\te}$ is of size $\left(\ell_{\max}+1\right)^2\times \left(\ell_{\max}+1\right)^2$ whose $\left( \ell_0m_0, \ell'm'\right)^{\mathrm{th}}$ entry is given by
\begin{align}\label{eq:definition_of_P_matrix}
\left[ \bP \chi_j^{\te}\right]_{\ell_0m_0}^{\ell'm'} &:= \sum_{n=1}^{N_{\leb}}\omega_n\chi_j^{\te}(\bx_j+R_j\bs_n)Y_{\ell_0m_0}(\bs_n)Y_{\ell'm'}(\bs_n).
\end{align}
Finally, we have the right-hand side vectors.  The $(i\ell m)^{\mathrm{th}}$ entry of the vector $\overline{\bG}_0$ is given by
\begin{equation}\label{eq:definition_of_G_0}
\left[ \overline{\bG}_0\right]_{i\ell m}=-\sum_{n=1}^{N_{\leb}}\omega_n \chi_i^{\te}(\bx_i+R_i\bs_n)\psi_0(\bx_i+R_i\bs_n)Y_{\ell m}(\bs_n).
\end{equation}
The $(i\ell m)^{\mathrm{th}}$ entry of $\overline{\bF}_0$ is given by
\begin{equation}\label{eq:definition_of_F_0}
\left[\overline{\bF}_0\right]_{i\ell m}=-\left(\sum_{n=1}^{N_{\leb}}\omega_n^{\leb}\chi_i^{\te}(\bx_i+R_i\bs_n)Y_{\ell m}(\bs_n)\sum_{j=1}^M\left[\bS\right]_{jin} \right),
\end{equation}
where
\begin{equation}\label{eq:defintion_of_S}
\left[\bS\right]_{jin}= \sum_{\ell_0=0}^{\ell_{\max}}\sum_{m_0=-\ell_0}^{\ell_0}\cik \clomo\bk_{\ell_0}^j(\bx_i+R_i\bs_n)Y_{\ell_0m_0}^j(\bx_i+R_i\bs_n),
\end{equation}
and
\begin{equation}\label{eq:definition_of_c_0_l_0_m_0}
\clomo=\sum_{n=1}^{N_{\leb}}\omega_n^{\leb} \chi_j^{\te}(\bx_j+R_j\bs_n)\partial_{\bn}\psi_0(\bx_j+R_j\bs_n)Y_{\ell_0m_0}(\bs_n).
\end{equation}

\begin{remark}
The matrix $\overline{\bC}_1, \overline{\bC}_2$, and $\overline{\bF}_0$ corresponding to $\bG_X$ are denoted by $\bC_1, \bC_2$, and $\bF_0$, respectively. Here $\bC_1$ is of dimension $MN\left(\ell_{\max}+1\right)^2\times MN\left(\ell_{\max}+1\right)^2$, $\bC_2$ is of dimension $MN\left(\ell_{\max}+1\right)^2\times M\left(\ell_{\max}+1\right)^2$ and $\bF_0$ is a column vector of size $MN\left(\ell_{\max}+1\right)^2$.
\end{remark}

\subsubsection{Linear Solver}
We finally obtain a system of equations of the form
$$
\begin{bmatrix}
\bA+\bC_1 & \bC_2\\
\overline{\bC}_1 & \bB+\overline{\bC}_2
\end{bmatrix}
\begin{bmatrix}
X_{\mr}\\
X_{\me}
\end{bmatrix}=
\begin{bmatrix}
\bG_0 + \bF_0\\
\overline{\bF}_0
\end{bmatrix},
$$
where matrix $\bA,\bB$ are sparse in nature, and $\bC_1,\bC_2$ (and $\overline{\bC}_1,\overline{\bC}_2$) are dense. Once can use a direct solver such as LU (or an iterative solver such as GMRes) to solve the above system of equations.  But, because of the dense nature of the matrix $\bC_1$ and $\bC_2$ the direct solvers are computationally inefficient. We introduced the global strategy in Sec.~\ref{sec:global_strategy} and hence we have an iterative process
$$
\begin{bmatrix}
\bA & 0\\
0 & \bB
\end{bmatrix}
\begin{bmatrix}
X_{\mr}^{(\tk)}\\
X_{\me}^{(\tk)}
\end{bmatrix}=
\begin{bmatrix}
\bG_0 + \bF_0\\
\overline{\bF}_0
\end{bmatrix}-
\begin{bmatrix}
\bC_1 & \bC_2\\
\overline{\bC}_1 & \overline{\bC}_2
\end{bmatrix}
\begin{bmatrix}
X_{\mr}^{(\mk-1)}\\
X_{\me}^{(\mk-1)}
\end{bmatrix},
$$
where $(\mk)$ denotes the outer iteration and $X_{\mr}^{(\mk)}$, $X_{\me}^{(\mk)}$ denote the solution at the $(\mk)^{\ith}$ step. In our simulations we update the RHS using the $(\mk-1)^{\ith}$ solution and then solve the system using a GMRes solver. The GMRes iteration are referred as inner iterations and the global iterations as outer iterations.

\begin{remark} To simplify the analysis we introduced a linearisation of $\mathcal{F}(\beta(\cdot))$ in Remark~\ref{rem:linear}. We give some details about this here. We see that the matrix $\bA^j$ is solution dependent for each $j$. Hence, to solve the global system 
$$
\bA\left(X_{\mr}^{(\mk)}\right)X_{\mr}^{(\mk)}=\left(\bG_0+\bF_0\right)-\left(\bC_1 X_{\mr}^{(k-1)}+\bC_2 X_{\me}^{(k-1)}\right),
$$
we need to solve the inner iteration using a fixed point. Let us for simplicity drop the $(\mk)^{\ith}$ iteration index and represent the above system by
$$
\bA\left(X\right)X=\bG.
$$
We solve this using a simple fixed-point
$$
\bA\left(X^{(\nu-1)}\right)X^{(\nu)}=\bG,
$$
where $(\nu)$ is referred as fixed-point (FP) iterations. The right-hand side $\bG$ depends on the $(\mk-1)^{\ith}$ solution which remains fixed throughout the FP-iteration loop.
\end{remark}

\begin{remark}\label{rem:intergtation_torus}
The final thing remaining in the discretisation process is the evaluation of the integrals in $\left[\bA^i\right]$. We have integrals over the torus $\mathcal{D}_i$ and the boundary of $B_{\delta_i}(\bx_i)$. Here we follow the ideas from \cite{QSM18}. For simplicity we take the example of unit ball. The integral over $\partial B_{\delta}(\bo)$ is given by
\begin{equation*}
\begin{aligned}
\frac{\ell}{\delta}\int_{\partial B_{\delta}(\bo)}\tilde{L}_i\ylmdash\tilde{L}_j\ylm &= \ell\delta \tilde{L}_i(\delta)\tilde{L}_j(\delta)\int_{\mathbb{S}^2}\ylm \ylmdash\\
& = \ell \delta \tilde{L}_i(\delta)\tilde{L}_j(\delta)\delta_{\ell \ell'}\delta_{m m'}.
\end{aligned}
\end{equation*}
The integral over $\mathcal{D}$ can be divided into two parts, radial and spherical. Let $h\in \mathcal{L}^{1}\left(B_1(\bo)\right)$ then the integral of $h$ over $\mathcal{D}$ can be written separately as
$$
\int_{\mathcal{D}}h(\bx)d\bx=\int_{\delta}^1r^2\int_{\mathbb{S}^2}h(r,\bs)d\bs dr,\quad \bs\in \mathbb{S}^2,
$$
and $\bx=r\bs$. The spherical part can be computed using Lebedev formula. For the radial part we use the Legendre-Gau\ss-Lobatto (LGL) quadrature rule \cite{Par99} defined by quadrature points $x_{m}\in [-1,1]$ and the quadrature weights $\omega_m^{\lgl}$, $1\leq m\leq N_{\lgl}$ for $N_{\lgl}$ quadrature points. Using change of variable
$$
r=\frac{1-\delta}{2}\left(x+1\right)+\delta,\quad x\in [-1,1],
$$
we approximate the integral by the following quadrature rule
$$
\int_{\mathcal{D}}h(\bx)d\bx\approx \frac{1-\delta}{2}\sum_{m=1}^{N_{\lgl}}\sum_{n=1}^{N_{\leb}}\omega_m^{\lgl}\omega_n^{\leb}\left(\frac{1-\delta}{2}(x_m+1)+\delta\right)^2h\left(\frac{1-\delta}{2}(x_m+1)+\delta,\bs_n\right).
$$
\end{remark}

==> effect_of_disc_parameter.tex <==
In example~\ref{subsec:gsp_solver}, we showed the effects of the discretization parameters $N$ and $N_{\lgl}$ for a one-atom system. Here in this example, we show it for the spherical parameters $\ell_{\max}$ and $N_{\leb}$ along with $N$ and $N_{\lgl}$ for the hydrogen-fluoride molecule. We start with an exact solution obtained for $\ell_{\max}=15$, $N_{\leb}=2354$, $N=25$, and $N_{\lgl}=50$. The geometric parameters are $r_p=1.5$\AA, $r_0=1$\AA, and $a=0.5$ \AA.

Fig.~ present results for the varying radial discretization parameters, i.e., $N$ (left) and $N_{\lgl}$ (right). We vary $N$ from $5$ to $20$ with keeping $N_{\lgl}=50$. For the LGL nodes, we vary from $25$ to $40$ with keeping $N=20$ fixed. The spherical discretisation parameters are set to $\ell_{\max}=15$ and $N_{\leb}=1454$. Similarly to example~\ref{subsec:gsp_solver}, we observe that our solvation energy improves when we use a higher degree of radial approximation.

Fig.~ present results for the spherical discretisation parameters, $\ell_{\max}$ (left) and $N_{\leb}$ (right). We set the radial parameters as $N=20$ and $N_{\lgl}=50$. We vary $\ell_{\max}$ from $3$ to $15$ by keeping $N_{\leb}=1454$ and similarly vary $N_{\leb}$ from $350$ to $4334$ while keeping $\ell_{\max}=15$. We notice that the approximations are improved as we increase the discretization parameters.

Convergence reached with 15 total iterations and Es       : -0.000619373
Convergence reached with 15 total iterations and Essol   : -0.000619374
Convergence reached with 15 total iterations and Esions  : 0.000601509
Convergence reached with 15 total iterations and Osmotic  : 0.000601508


==> effect_of_stern.tex <==
In this example, we want to study the effect of the Stern layer on the electrostatic solvation energy. For this, we consider the hydrogen-fluoride molecule with the discretization parameter $\ell_{\max}=9$, $N_{\leb}=350$, $N=10$, and $N_{lgl}=20$. We keep the probe radius fixed as $1.5$ \AA and vary the Stern layer from $0$ to $1$ \AA. To keep the layer's width $\mathcal{L}$ fixed, we set $r_0=1-a$ \AA. The purpose of the ion-exclusion function is to exclude the ions near $\Omega_{\ses}$. The smaller the Stern layer length, one would assume less electrostatic solvation energy.

Fig.~\ref{fig:energy_parameter_a} presents different solvation energies for varying $a$. We notice that as $a$ is increased $E_s$ (top left) and $E_s^{\sol}$ (bottom) decreases monotonically. The energy contribution from $\rho^{\ions}$, i.e., $E_s^{\ions}$ (top right) attains its minimum at $a=0.5$ \AA, and hence throughout the studies, we consider this parameter.

\input{figures/relative_discretisation_parameter_a.tex}

==> old_numres.tex <==
In this section we present some numerical results for the ddPB method.

\subsection{GSP Solver Test}
We start with the test of the GSP solver that was developed in Sec.~\ref{sec:single_domain}. We consider a single atom molecule with unit charge centred at the origin, with the vdW radius,  $r_i=0.5$. We set the SAS probe radius, $r_p=0.3$, and the Stern layer length, $a=0.2$. With only one atom the spherical part of the molecule can be neglected and hence only the radial part contributes.

Regarding the dielectric permittivity, we consider $\varepsilon_s=10$ and the smoothing function
$$
\xi(t)=1+\left(\varepsilon_s-1\right)t^3\left(10+3t(-5+2t)\right),\quad 0\leq t\leq 1.
$$

To compute the results, unless mentioned we set the default discretisation parameters as, $\ell_{\max}=6$, $N=20$, $N_{\lgl}=50$, and $N_{\leb}=100$.  Finally, we set the Debye-H\"uckel constant as $1$ and $\beta=1$.

To compare the results we introduce the energy function, $E_s$ which is computed by
$$
E_s=\frac{1}{2}\langle \psi_{\mr}, \rho^{\sol}-  \rho^{\mathrm{ions}}\rangle.
$$
As we are dealing with one atom the above formulation reduces to 
$$
E_s=\sum_{n=1}^{N_{\leb}}q_1\omega_n^{\leb}\psi_r(\bs_n)Y_{0,0}(\bs_n).
$$

We first present results by varying the non-linear region which is controlled by the parameter $r_0$ for $r_0\in \lbrace 0.5, 1, 1.5, 2, 2.5, 3, 3.5, 4, 4.5, 5.0,10\rbrace$.  Fig.~\ref{fig:solvation_varying_r0} shows the solvation energy with varying $r_0$. Table~\ref{tab:energy_non_linear_varying_r0} presents the non-linear iteration and the energy for the same.

\begin{table}
\centering
\begin{tabular}{|c|c|c|}
\hline
$r_0$ & $E_s$ & $N_{\mathrm{ite}}$\\
\hline\hline
0.5 & -0.55717 &  5\\
1.0 & -1.0153 & 6\\
1.5 & -1.2499 & 7\\
2.0 &  -1.2824 & 9\\
2.5 & -1.2255 & 10 \\
3.0 & -1.1818 & 11 \\
3.5 & -1.121 & 12 \\
4.0 & -1.096 & 13\\
4.5 & -1.0652 & 14\\
5.0 & -1.027 & 15\\
10 & -1.8385 & 64\\
11 & -2.4947 & 97\\
\hline
\end{tabular}
\caption{Energy and number of non-linear loops for one atom with respect to varying $r_0$.}\label{tab:energy_non_linear_varying_r0}
\end{table}


Next, we plot the error function with respect to $N$, where
$$
\mathtt{Error}(N)=|E_s^N-E_s^{\infty}|,
$$
where $E_s^{\infty}$ is obtained with $r_0=1.5$, $\ell_{\max}=6$, $N_{\lgl}=100$, and $N=30$, Fig.~\ref{fig:error_es_varying_N}.

Now, we plot the $\ell^2$-error of the solution with respect to $N$, i.e., $\|u^{\infty}-u^n\|_{\ell_2}^2$ where $u^{\infty}$ is obtained with $N=30$, $r_0=1$, and $N_{\lgl}=100$, Fig.~\ref{fig:l2_error_N}.

\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
    legend pos=north east, xlabel = \Large{$N$}, ylabel= \Large{$\mathtt{Error}(N)$},     legend cell align ={left}, title = {\Large{Error vs $N$}}]
\addplot[color=blue,  mark=square*, line width = 0.5mm, dashdotted,, mark options = {scale= 1.0, solid}] 
coordinates{(5, 0.0216281118)(7,0.0223984980)(10, 0.0628972947)(12,0.0643093702)(15,0.0369605293)(17,0.0161030506)(20, 0.0061993340)(22, 0.0001769156)(25, 0.0058703508)(27,0.0068682544)};
\end{axis}
\end{tikzpicture}
\caption{Error plots for varying $N$.}\label{fig:error_es_varying_N}
\end{figure}
 
\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
    legend pos=north east, xlabel = \Large{$r_0$}, ylabel= \Large{$E_s$},     legend cell align ={left}, title = {\Large{Solvation Energy}}]
\addplot[color=blue,  mark=square*, line width = 0.5mm, dashdotted,, mark options = {scale= 1.0, solid}] 
coordinates{(0.5, -0.55717)(1.0, -1.0153)(1.5, -1.2499)(2.0, -1.2824)(2.5, -1.2255)(3.0 ,-1.1818)(3.5, -1.121)(4.0, -1.096)(4.5,  -1.0652)(5.0, -1.027)(10, -1.8385)(11, -2.4947) };
\end{axis}
\end{tikzpicture}
\caption{Solvation Energy with varying $r_0$.}\label{fig:solvation_varying_r0}
\end{figure}

\begin{table}
\centering
\begin{tabular}{|c|c|c|}
\hline
$a$ & $E_s$ & $N_{\mathrm{ite}}$\\
\hline\hline
0.1 & -0.869092 &  5\\
0.3 & -1.104819 & 6\\
0.5 & -0.918014 & 7\\
0.7 &  Oscillate & -\\
1.0 & NaN & - \\
\hline
\end{tabular}
\caption{Energy and number of non-linear loops for one atom with respect to varying Stern layer length, $a$.}
\end{table}

\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
    legend pos=north east, xlabel = \Large{$N$}, ylabel= \Large{$\|u^{\infty}-u_n\|^{\ell_2}$},     legend cell align ={left}, title = {\Large{$\ell^2$- Error}}]
\addplot[color=blue,  mark=square*, line width = 0.5mm, dashdotted,, mark options = {scale= 1.0, solid}] 
coordinates{(5, 32.0304)(10, 19.4829)(15,12.1516)(20, 7.0633)(25, 3.1817)};
\end{axis}
\end{tikzpicture}
\caption{$\ell^2$-error plots for varying $N$.}\label{fig:l2_error_N}
\end{figure}
 


==> vis_reaction_potential.tex <==
In this example, we visualize the reaction potential on the enlarged cavity $\Omega_0$. Fig.~\ref{fig:reaction_potential_hf_ch4} shows the reaction potential for hydrogen-fluoride (left) and the formaldehyde (right) molecule, respectively, with the discretization parameter $\ell_{\max}=11$, $N_{\leb}=1202$, $N=15$, and $N_{\lgl}=50$. The geometric parameters are set to $r_p=1.5$ \AA, $r_0=1$ \AA, and $a=0.5$\AA. We observe the rotational symmetry for the hydrogen-fluoride molecule and the mirror symmetry for the formaldehyde molecule.

\begin{figure}[t!]
\centering
\includegraphics[scale=0.1]{figures/hf_pot.jpg}\hspace*{5em}
\includegraphics[scale=0.1]{figures/formaldehyde_pot.jpg}
\caption{Example~\ref{subsec:vis_reac_pot}: Reaction potential for hydrogen-fluoride molecule (left) and formaldehyde molecule (right) on $\Omega_0$. 
}\label{fig:reaction_potential_hf_ch4}
\end{figure}

Fig.~\ref{fig:reaction_potential_caffeine} presents results for the caffeine molecule with 24 atoms. Here we use the discretization parameters $\ell_{\max}=9$, $N_{\leb}=350$, $N=15$, and $N_{\lgl}=30$.  The geometric parameters are set similarly to the previous molecules.

\begin{figure}[t!]
\centering
\includegraphics[scale=0.1]{figures/caffeine_pot.jpg}
\caption{Example~\ref{subsec:vis_reac_pot}: Reaction potential for caffeine on $\Omega_0$. 
}\label{fig:reaction_potential_caffeine}
\end{figure}


